Ramsey-type problems in orientations of graphs

Given an acyclic oriented graph $\vec{H}$ and a graph $G$, we write $G \to \vec{H}$ if every orientation of $G$ has an oriented copy of $\vec{H}$. We define $\vec{R}(\vec{H})$ as the smallest number $n$ such that there exists a graph $G$ satisfying $G \to \vec{H}$. Denoting by $R(H)$ the classical Ramsey number of a graph $H$, we show that $\vec{R}(\vec{H}) \leq 2R(H)^{c \log^2 h}$ for every acyclic oriented graph $\vec{H}$ with $h$ vertices, where $H$ is its underlying undirected graph. We also study the threshold function for the event $\{G(n,p) \to \vec{H}\}$ in the binomial random graph $G(n,p)$. Finally, we consider the isometric case, in which we require that, for every two vertices $x, y \in V(\vec{H})$ and their respective copies $x', y'$ in $\vec{G}$, the distance between $x$ and $y$ is equal to the distance between $x'$ and $y'$. We prove an upper bound for the isometric Ramsey number of an acyclic orientation of the cycle, applying the hypergraph container lemma in random graphs.

==> abstract <==
Given an acyclic oriented graph $\vec{H}$
and a graph $G$,
we write
$G \to \vec{H}$
if
every orientation of $G$
has an oriented copy of
$\vec{H}$.
We define
$\dr(\dgh)$
as the smallest number $n$ such that there exists a graph
$G$ satisfying $G \rms \dgh$.
% Applying a result of 
% Conlon, Fox, Lee, Sudakov~\cite{conlon_ordered},
Denoting by $R(H)$
the classical Ramsey number of a graph $H$,
we show that
$\dr(\dgh) \leq 2R(H)^{c \log^2 h}$
for every acyclic oriented graph $\dgh$ with $h$ vertices,
where $H$ is its underlying undirected graph.
We also study the threshold function for
% this problem
the event 
$\{G(n,p) \rms \dgh\}$
in the binomial random graph $G(n,p)$.
Finally, we 
consider
the
% \emph{isometric} 
{isometric} 
case,
in which we require 
that,
for every two vertices
$x, y \in V(\dg{H})$
and their respective copies
$x', y'$
in $\dg{G}$,
the distance between $x$ and $y$
is equal to the distance
between $x'$ and $y'$.
We prove an upper bound for the
isometric Ramsey number of an acyclic orientation of the
cycle, applying the hypergraph container lemma in random
graphs.
% adapting an argument of
% {H{\`a}n},
% {Retter},
% {R{\"o}dl}
% and
% {Schacht}~\cite{han_ramsey_containers}.
\end{abstract}


